Index problems for game automata

For a given regular language of infinite trees, one can ask about the minimal number of priorities needed to recognize this language with a non-deterministic, alternating, or weak alternating parity automaton. These questions are known as, respectively, the non-deterministic, alternating, and weak Rabin-Mostowski index problems. Whether they can be answered effectively is a long-standing open problem, solved so far only for languages recognizable by deterministic automata (the alternating variant trivializes). We investigate a wider class of regular languages, recognizable by so-called game automata, which can be seen as the closure of deterministic ones under complementation and composition. Game automata are known to recognize languages arbitrarily high in the alternating Rabin-Mostowski index hierarchy; that is, the alternating index problem does not trivialize any more. Our main contribution is that all three index problems are decidable for languages recognizable by game automata. Additionally, we show that it is decidable whether a given regular language can be recognized by a game automaton.

==> aut_restr_fig.tex <==
\usetikzlibrary{calc}

\begin{tikzpicture}
\tikzstyle{edge}=[draw, thick, ->]

\coordinate (zero) at (0,0);

\path[draw=black, rounded corners=5] ($(zero)+(0,0)$) rectangle ($(zero)+(2,-3)$);

\path[draw=black, rounded corners=5] ($(zero)+(2.3,0)$) rectangle ($(zero)+(3.3,-3)$);

\node at ($(zero)+(1,0.4)$) {$Q$};
\node at ($(zero)+(2.8,0.4)$) {$F$};

\foreach \y in {1,...,4} {
  \draw[edge] ($(zero)+(1.8, 0.5-\y*0.8)$) -- ++(0.7,0);
}

\foreach \x in {1,...,2} {
  \draw[edge] ($(zero)+(\x*0.4,-1.15)$) -- ++(0,-0.7);
}

\foreach \x in {1,...,2} {
  \draw[edge] ($(zero)+(2-\x*0.4,-1.85)$) -- ++(0,0.7);
}


\coordinate (cu0) at ($(zero)+(1.0,-0.6)$);

\draw[edge] ($(cu0)+(0,0.3)$) arc (90:-90:0.3);
\draw[edge] ($(cu0)-(0,0.3)$) arc (90:-90:-0.3);

\coordinate (cu1) at ($(zero)+(1.0,-2.4)$);

\draw[edge] ($(cu1)+(0,0.3)$) arc (90:-90:0.3);
\draw[edge] ($(cu1)-(0,0.3)$) arc (90:-90:-0.3);

\draw[dotted] ($(zero)+(0,-1.5)$) -- ($(zero)+(2,-1.5)$);


\coordinate (zero) at (5,0);

\path[draw=black, rounded corners=5] ($(zero)+(0,0)$) rectangle ($(zero)+(2,-1.35)$);

\path[draw=black, rounded corners=5] ($(zero)+(2.3,0)$) --
	++(1.0,0) --
    ++(0,-3) --
    ++(-3.3,0) --
    ++(0,1.35) --
    ++(2.3,0) -- cycle;

%rectangle ($(zero)+(3.3,-3)$);

\node at ($(zero)+(1,0.4)$) {$Q'$};
\node at ($(zero)+(2.8,0.4)$) {$F'$};

\foreach \y in {1,...,2} {
  \draw[edge] ($(zero)+(1.8, 0.5-\y*0.8)$) -- ++(0.7,0);
}

\foreach \x in {1,...,2} {
  \draw[edge] ($(zero)+(\x*0.4,-1.15)$) -- ++(0,-0.7);
}

\coordinate (cu0) at ($(zero)+(1.0,-0.6)$);

\draw[edge] ($(cu0)+(0,0.3)$) arc (90:-90:0.3);
\draw[edge] ($(cu0)-(0,0.3)$) arc (90:-90:-0.3);

\end{tikzpicture}

